Pros and Cons! Evaluating ChatGPT on Software Vulnerability

This paper proposes a pipeline for quantitatively evaluating interactive LLMs such as ChatGPT using publicly available dataset. We carry out an extensive technical evaluation of ChatGPT using Big-Vul covering five different common software vulnerability tasks. We evaluate the multitask and multilingual aspects of ChatGPT based on this dataset. We found that the existing state-of-the-art methods are generally superior to ChatGPT in software vulnerability detection. Although ChatGPT improves accuracy when providing context information, it still has limitations in accurately predicting severity ratings for certain CWE types. In addition, ChatGPT demonstrates some ability in locating vulnerabilities for certain CWE types, but its performance varies among different CWE types. ChatGPT exhibits limited vulnerability repair capabilities in both providing and not providing context information. Finally, ChatGPT shows uneven performance in generating CVE descriptions for various CWE types, with limited accuracy in detailed information. Overall, though ChatGPT performs well in some aspects, it still needs improvement in understanding the subtle differences in code vulnerabilities and the ability to describe vulnerabilities in order to fully realize its potential. Our evaluation framework provides valuable insights for further enhancing ChatGPT' s software vulnerability handling capabilities.

==> sections/insights_takeaways.tex <==
\section{Insights and Takeaways}

After analysis and discussion by task, we have some insights and takeaways to provide to subsequent researchers.


\begin{itemize}
    \item ChatGPT demonstrates varied detection capabilities for different CWE types, excelling in detecting ``NULL Pointer Dereference'' and the ``Permissions, Privileges, and Access Controls''  vulnerabilities (i.e., CWE-476 and CWE-264), while struggling with authorization checking, resource management, and input validate checking related vulnerabilities (i.e., CWE-200, CWE-20, CWE-399, and CWE-41).
    \item ChatGPT lacks confidence in vulnerability detection and can be easily induced to change its decision, particularly when classifying vulnerable functions.
    \item ChatGPT's vulnerability assessment ability is strong and stable overall, but its performance varies across different classes and can be weakened by providing key information.
    \item ChatGPT's capability in locating vulnerabilities is influenced by the specific CWE category being analyzed, with varying performance across different types.
    \item ChatGPT's effectiveness in fixing code vulnerabilities varies across different classes and is influenced by the class of vulnerability, with the additional context of vulnerable related lines generally improving performance, although the impact of context is inconsistent across classes.
    \item ChatGPT exhibits a moderate level of similarity between generated descriptions and ground truth, with varying performance across vulnerability categories and robustness in handling diverse data, especially the “Other” category.
\end{itemize}
